Inferring Facing Direction from Voice Signals

Consider a home or office where multiple devices are running voice assistants (e.g., TVs, lights, ovens, refrigerators, etc.). A human user turns to a particular device and gives a voice command, such as ``Alexa, can you ...''. This paper focuses on the problem of detecting which device the user was facing, and therefore, enabling only that device to respond to the command. Our core intuition emerges from the fact that human voice exhibits a directional radiation pattern, and the orientation of this pattern should influence the signal received at each device. Unfortunately, indoor multipath, unknown user location, and unknown voice signals pose as critical hurdles. Through a new algorithm that estimates the line-of-sight (LoS) power from a given signal, and combined with beamforming and triangulation, we design a functional solution called CoDIR. Results from $500+$ configurations, across $5$ rooms and $9$ different users, are encouraging. While improvements are necessary, we believe this is an important step forward in a challenging but urgent problem space.

==> tex/algo_temp.tex <==

\begin{algorithm}[htb]
\caption{\hl{Facing Direction} $(x_{ij})$ }
\begin{algorithmic}
\STATE $X_{i} = DelaySumAoA (x_{i1}, x_{i2} ... x_{iM})$ 

\STATE $\hat{v}^{0} = AlignCorrelate (X_{1}, X_{2} ... X_{N})$ 

\STATE $j=0$

\WHILE{$|\hat{v}^{j}-\hat{v}^{j-1}|>\Delta$}
\STATE $h_{i}^{j} = Deconvolve (X_{i}, \hat{v}^{j})$

\STATE $h = PeakAlign (h_{1}^{j,+}, h_{2}^{j,+} ... h_{N}^{j,+})$ 

\STATE $\hat{v}^{j+1} = Deconvolve (\hat{v}^{j}, h)$
\STATE $j=j+1$
\ENDWHILE
%\STATE $i\gets 10$
%\IF {$i\geq 5$} 
%        \STATE $i\gets i-1$
%\ELSE
%        \IF {$i\leq 3$}
%                \STATE $i\gets i+2$
%        \ENDIF
%\ENDIF 
\end{algorithmic}
\label{alg:fd}
\end{algorithm}


==> tex/core_algo.tex <==

\section{The {\name} Algorithm}
This section presents our proposed algorithm for extracting $P^{(LoS)}_{i}$ from the received signal $x_{ij}$.
We focus on the core technique, assuming the other modules (like device and user localization) are solved.
The next section will discuss those modules and pull together the end to end {\name} system.

\subsection{Intuition}
Let us begin with a high level intuition -- this will not explain the algorithm but should show the line of thinking. 
Our aim is to harness the maximum amount of diversity gain possible, and therefore use all $N\times M$ microphones together.
Although the powers $P^{(LoS)}_{i}$ are very different across the $N$ devices, the source voice signal is the same in all of them.
If we can reasonably estimate the source signal (i.e., estimated $\hat{v}(t)$ is in the neighborhood of the true voice signal $v(t)$), 
then it might be possible to estimate channels $\hat{h}_{ij}$ that are also in the neighborhood of the true channel $h_{ij}$.
Now, if we diversity-combine the channels, we expect to estimate a better source signal (closer to $v(t)$), 
and in turn a better channel estimate\footnote{Since convolution is linear, combining the received signals is the same as first 
combining the channels and then convolving with the source signal.}.
Iteratively, we expect both the source signal and the channel to converge.
%, terminating when they don't change any more.
At this point, the first channel tap in each of $\hat{h}_{ij}$ should correspond to the LoS component, which should lead us to $P^{(LoS)}_{i}$.
Let us now explain the actual algorithm. 

\subsection{Primitives}
We first define two primitives, as visualized in Figure \ref{fig:primitives}.
\new

% Primitive definition
\textbf{Delay and Sum on AoA - $\sum^{AoA}$}: 
Align the signals from multiple microphones on the same device according to signal AoA.
Each device records $M$ microphone signals and combines them to form a clean $X_{i}$.
Given the device and user locations, the AoA $\theta_i$ from the user to device $D_i$ is known.
The device aligns the received signals $x_{ij}$ from all microphones according to $\theta_i$, obtaining
$X_{i} = \sum^{AoA}_j x_{ij}$. Here we define 
\minus
\begin{align*}
    \sum\nolimits^{AoA}_j x_j(t)&\coloneqq \sum_j x_{j}(t-\Delta_j)\\
    \Delta_j &= \vec{m_j}\cdot\vec{\theta_i}/V_s
\end{align*}
where $\Delta_j$ is the AoA delay of microphone $m_j$, and
$\vec{m_j}$ and $V_s$ denote the $m_j$'s placement and sound-speed respectively.

\begin{figure}[hbt]
\centering
\includegraphics[width=3.2in]{figs/algoPrimitives.pdf}
\minus \minus
\caption{Basic primitives for the {\name} algorithm.}
\label{fig:primitives} 
\vspace{-0.05in}
\end{figure}

\textbf{Align on correlation - $\sum^{Corr}$}:
Align signals received from different devices of the same speech with cross correlation.
It first aligns the strongest multipath components, which may be the LoS component,
in each device channel, and creates a signal $\hat{v}$. 
$\hat{v}$ features strong single tap channel, which is close to the 
source signal. We define 
\begin{align*}
    \sum\nolimits^{Corr}_j x_j(t)\coloneqq \sum_j x_{j}(t-\delta_j)
\end{align*}
where $\delta_j = {argmax}_{\delta} (corr(x_0(t),x_j(t-\delta)))$.

\subsection{Algorithm}
Algorithm \ref{alg:fd} presents the pseudo code for {\name}, so let's zoom into the details.
% Set expectation : how many steps ? 
There are five steps in the algorithm. 
\new

% Construct X_i
\textbf{Step 1: Each device aligns signals}: 
Each device $D_i$ computes a single channel signal 
$X_{i} = \sum^{AoA}_j x_{ij}$ from microphones $m_{ij}$, $j\in[1,M]$. 
By aligning signals according to the AoA of the user, we can slightly 
eliminates ambient noises and multipath effects from other directions, and mitigate
 thermal noises from the microphones.
\new

\begin{algorithm}[t]
\caption{Facing Direction $(x_{ij})$ }
\begin{algorithmic}
\STATE $X_{i} = DelaySumAoA (x_{i1}, x_{i2} ... x_{iM})$ 

\STATE $\hat{v}^{0} = AlignCorrelate (X_{1}, X_{2} ... X_{N})$ 

\STATE $j=0$

\WHILE{$|\hat{v}^{j}-\hat{v}^{j-1}|>\Delta$}
\STATE $h_{i}^{j} = Deconvolve (X_{i}, \hat{v}^{j})$

\STATE $h = PeakAlign (h_{1}^{j,+}, h_{2}^{j,+} ... h_{N}^{j,+})$ 

\STATE $\hat{v}^{j+1} = Deconvolve (\hat{v}^{j}, h)$
\STATE $j=j+1$
\ENDWHILE
%\STATE $i\gets 10$
%\IF {$i\geq 5$} 
%        \STATE $i\gets i-1$
%\ELSE
%        \IF {$i\leq 3$}
%                \STATE $i\gets i+2$
%        \ENDIF
%\ENDIF 
\end{algorithmic}
\label{alg:fd}
\end{algorithm}

% Construct \hat{v}^0
\textbf{Step 2: Construct initial signal estimation $\hat{v}^0$}: 
The signal from each device $X_i$ is shared with the leader device.
The leader device then aligns these signals together to compute 
the first estimation of the source signal $\hat{v}^0(t)$. 
\begin{align}
    \hat{v}^0 &= \sum\nolimits^{corr}_i X_i &= \sum\nolimits^{corr}_i v*h_i &= v*\sum\nolimits^{corr}_i h_i
    \label{eq:est_v}
\end{align}

% Explain why \hat{v}^0 is a nice estimation
% Because we want strongest delta component
Consider the mixed channel $h = \sum^{corr}_i h_i$, 
if we assume that channels of the devices are uncorrelated with each others.
The align on correlation will align and add up the strongest multipath components
 constructively from every channel. 
Accordingly, we have
\begin{align*}
    \sum\nolimits^{corr}_i h_i(t) &= \sum_i h_i(t-argmax(h_i))\\
    max(h) &= \sum_i max(h_i) 
        \minus
\end{align*}
The maximal tap of channel $h$ is $N$ times larger than $h_i$, 
while other taps in $h_i$ are added up less as channels are uncorrelated.
This sharpened channel, in which maximal tap is much higher than others, 
is of high SNR, low multipath and make the aligned signal 
$\hat{v}^0$ a good estimation of $v$.
\new

\begin{figure*}[hbt]
\minus \minus
\centering
\includegraphics[width=2.2in, height=1.5in]{figs/dummy.pdf}
\hfill
\includegraphics[width=2.2in, height=1.5in]{figs/dummy.pdf}
\hfill
\includegraphics[width=2.2in]{figs/circularCorrelation.pdf}
\minus \minus
\caption{(a) Simulation of convergence of algorithm. (b) Simulation with gaussian signal. (c) Correlating equalized powers from devices (red arrows) with human radiation pattern (black and time-shifted gray lines).}
\label{fig:correlate} 
\vspace{-0.05in}
\end{figure*}

\textbf{Step 3: Estimate $h_i$ and $h$ from $\hat{v}$}: 
Given the estimated source signal $\hat{v}$, we can estimate the 
 device channel $h_i$ by deconvolution. 
The estimated channel is obtained by $\hat{h}_i^0=deconvolve(X_i,\hat{v}^0)$ 
and the estimated mixed channel $h$ can be calculated as 
$\hat{h}^0=\sum^{corr}_i \hat{h}_i^{0,+}$, where $\hat{h}_i^{0,+}$ 
only preserves the positive values of $\hat{h}_i$ and make taps of negative 
amplitudes zero.
\new

From the mathematical perspective, removing negative parts of $\hat{h}_i$ makes the function none-linear, 
otherwise we will get $\hat{h}$ as the delta function 
\begin{align*}
    \sum\nolimits^{corr}_i \hat{h}_i &= \sum\nolimits^{corr} deconvolve(X_i, \hat{v}^0)\\
    &= \sum\nolimits^{corr}_i deconvolve(v*h_i, v*\sum\nolimits^{corr}_i h_i)\\
    &= deconvolve(\sum\nolimits^{corr}_i v*h_i, v*\sum\nolimits^{corr}_i h_i)\\
    &= \delta(t)
\end{align*}

\textbf{Step 4: Iteratively approximate $v$ from $\hat{v}^j$}:
We next target to approximate $v$ from our current estimation $\hat{v}^0$.
Recall that in Equation ~\ref{eq:est_v}, we know that the estimated source signal 
is the true signal convolve with the mixed channel $h$, of which we now have the estimation.
As a result, we can observe the better estimation of the source signal $\hat{v}^1$ by
 deconvolving $\hat{v}^0$ with $\hat{h}^0$, and start next iteration estimation
from \textbf{Step 3}.
\new

\textbf{Step 5: Stop and correlate LoS power with the radiation pattern}: 
\name\ finally predicts the facing direction from the estimated device channels.
The iterative algorithm stops when the channel estimation $\hat{v}$ converges, 
and the difference of estimated signal between two iterations is smaller than a 
threshold $\Delta$. 
We next take the estimated channel $\hat{h_i}^j$ of device $D_i$ after 
the $j$-th iteration and record the amplitude of the first peak $A_i$.
This amplitudes are used to calculate the LoS power 
$P_i^{LoS} = A_i^2$. $P_i^{LoS}$ is then 
equalized by the distance to the user $P_i^* = P_i^{LoS}\times d_i^2$.
\name\ next correlates the equalized power with radiation pattern facing each device,
and reports the facing device $D_k$ with the max correlation, as shown in 
Figure ~\ref{fig:correlate}. 
\begin{align*}
    k = {argmax}_i (corr(\mathbf{P^*},RP(i)))
\end{align*}
where $\mathbf{P^*}$ is the vector formed by equalized power $P_i^*$ from all the devices,
and $RP(i)$ is the radiation pattern facing device $D_i$. 
We show that speech radiation patterns are similar across different user,
 and using a universal radiation pattern does not affect the accuracy in 
Section ~\ref{sec:eval}.

% Estimate h_i from \hat{v}^0
% Estimate channel of delay and sum signal
% refine estimated signal


%$Y = \sum^{d} X_{i}$
%$X_{i} = \sum^{d} x_{ij} = v * \sum^{d} h_{ij}$
%\new


%Our core intuition is two-fold.
%(1) If the source signal is within some neighborhood of the true $v(t)$, the corresponding channel estimates will also lie in the neighborhood of the true channels $h_{ij}$.
%(2) Once we have reasonable channel estimates, diversity-combining them across many microphones can further improve the channel estimate, which can in turn improve the source signal estimate.



%Our core intuition is to harness the maximum amount of diversity gain possible, across $N$ devices and $MxN$ microphones.
%For this, we start by carefully combining all the $MxN$ microphone signals -- we expect the summed signal to be a first approximation of the source signal (i.e, the LoS component boosted over the multipath).
%% to achieve as much diversity combining gain as possible.
%%This must be done carefully since device are not clock synchronized.
%%If done correctly, the combined signal could be an approximation of the source signal (i.e., the LoS component boosted over the multipath).
%Now, pretending this first approximation source signal, say $\hat{v}^{(1)}(t)$, we estimate the channels at each device (via deconvolution).
%The channel estimates are of course inaccurate, but should boost the LoS channel tap (since the $\hat{v}^{(1)}(t)$ embeds a stronger LoS component).
%\new
%
%Now, in the key step of our algorithm, we align the LoS taps of the channels and sum them to further boost the LoS component.
%%se estimated channels to further boost the LoS tap (the alignment is for the LoS taps of the channel)
%Then, we use this combined channel to update the source signal, i.e., $x(t) = 
%This iteration continues, thereby jointly converging on to a better source signal and channel.
%
%\new



%\textbf{OLD TEXT BELOW} \\
%The core intuition with {\name} is to first carefully combine the signals from all the microphones (across all the devices) to obtain some estimate of the source signal.
%Now, believing that this is a good estimate of the source signal, {\name} estimates the channel expected at each device.
%Of course, these channel estimates would be incorrect to the extent the source signal is incorrect.
%So, to improve the channel estimates, {\name} combines the $N$ channels so that spurious channel taps are suppressed and the prominent ones are the actual channel taps experienced at different devices.
%Now, using this combined channel, it should be possible to update the source signal (we will see this mathematically soon).
%With the updated source signal, new channel estimates can be again derived, which leads to further improvements in the source signal.
%We expect this process to converge to a goos estimate of the source signal, and thereby a good estimate of the channel estimate at each device.
%For any given device, the amplitude of the first tap of the channel corresponds to the LoS path -- this is the value we are after.
%We derive the LoS signal power from this value, and then progress with distance-equalization and correlation steps as mentioned earlier.
%\new






==> tex/eval.tex <==
\section{Evaluation}
\label{sec:eval}

\subsection{Implementation}
Each of our ``devices'' is implemented on a Raspberry Pi4 ($64$ GB) \cite{RaspberryPi}, mounted with a $6$-microphone circular array from SEEED ReSpeaker \cite{ReSpeaker}.
Figure~\ref{fig:respeaker} shows complete device.
The arrangement of the microphones are similar to Amazon Echo or Google Home, but unlike these devices, the raw acoustic samples are available with the SEEED at $16,000$Hz.
The acoustic signals are piped to a native speech recognition system, which upon detecting wake-words like ``Alexa'' or ``Snowboy'', forwards the signal segment to {\name}.
The {\name} modules run on the Pi, and depending on whether a device is a follower or leader, signal information are transmitted/received.
Finally, the leader device computes the facing direction and notifies all the devices -- a green LED lights up on the facing device.

%the components of the device. We employ the 6 on-board mics as receiver of the acoustic signals and use the LED to indicate which device the user is facing towards. 
%The geometric arrangement of microphones on the Seeed 6-Mic Array is 
%similar to those of Google home and Amazon Echo, yet unlike the commercial devices, Seeed makes raw acoustic samples available to developers. 

\begin{figure}[hbt]
\centering
\includegraphics[width=0.8\columnwidth]{figs/eval/imp/Pi_dummy.JPG}
\caption{Receivers composed of 6-Mic circular array and Raspberry Pi4.}
\vspace{-0.15in}
\label{fig:respeaker}
\end{figure}



For P2P device localization -- where devices need to play short sounds -- we place a small XiaoMi Bluetooth speaker~\cite{XiaoMi} \hl{below each device.}
The sounds and data exchanges are coordinated by the leader device over WiFi (using socket connections).
The leader device \rui{functionalites is programmed in one script and all the devices used in our experiment has a copy of this. At run time, a leader device} is chosen arbitrarily, implying that any device can take on this role. \rui{There is possibly a marginal gain obtainable via optimizing which device to choose as the leader w.r.t its speed of the wireless connection, current load, location etc. We envision this task can be incorporated in a larger resource management framework orchestrating computational tasks in the vicinity, and we indeed provide the modularity and flexibility towards such incorporation.} Our overall framework is implemented in Python and is easily extensible to variations, such as BLE, Zigbee, or offloading to edge devices.

%We implement the proposed framework in python, and it will be available to public upon paper acceptance. We use an open source implementation of keyword detection and AoA detection is based on GCC-PHAT \cite{web:voiceengine}.

                    
\subsection{Experiment Methodology}
Our experiments are executed with $N=8$ devices, scattered in thousands of configurations across $5$ different rooms. 
We pretend that the devices are embedded in the environment (in TVs, thermostats, coffee machines, refrigerators, floor lights, etc.), hence often place them adjacent to such gadgets.
Figure~\ref{fig:rooms} shows $4$ rooms and a floorplan of the building, indicating that these are not controlled environments (instead are rich in multipath as would be the case in real homes and offices).
For voice commands, we recruit $9$ adult volunteers, almost equally divided between males and females, and ask them to speak while standing, seated, or even walking slowly.
Ground truth is measured using a laser ranger, so the locations of devices and volunteers are known to a millimeter resolution.
\new

During experimentation, we invite each volunteer to pick arbitrary locations in a room and speak the wake-word $8$ times, facing each device. 
From this data, we pick all subsets of $2$, $4$, and $6$ devices, and evaluate facing direction accuracy for these configurations.
This covers a wide range of scenarios -- some in which all devices are on one side of the user, while others in which the user is surrounded by devices.
These experiments are repeated over multiple configurations, rooms, and users.
Altogether, we record $2631$ audio clips resulting in $>5,000$ facing direction tests.
\new


\textbf{Success metric:}
We define two main metrics of evaluation, namely {\em Facing Direction Error (FDE)} and {\em Facing Integer Error (FIE)}.
Consider Figure \ref{fig:metric} where the user is truly facing $D_{i}$, and assume that {\name} determines $D_{k}$ as the facing device. In this case, $FDE=\theta$ and $FIE=2$ since $D_{k}$ is angularly separated by $2$ devices from $D_{i}$.
Now, if $D_{j}$ was not present, then FDE is still $\theta$ but FIE would now be $1$.
This captures that {\name} could not have done any better than $\theta$ since there is no other device less than $\theta$ degrees away.
\begin{figure}[h!]
\centering
\vspace*{-1.2em}
\includegraphics[width=0.7\columnwidth,trim= 0cm 0cm 0cm 0.8em,clip=true]{figs/metric4.pdf}
\caption{Facing direction error (FDE) and facing integer error (FIE) to characterize the nature of errors.}
\vspace{-0.15in}
\label{fig:metric}
%\vspace*{-1.2em}
\end{figure}
Of course, in addition to FDE and FIE, we will also measure user location errors, \hl{and other microbenchmarks like robustness across users, background sounds, user mobility, etc.}
\new
%\textbf{Success metric} is not only the accuracy of detecting the facing device, but also understanding the nature of errors (i.e., \hl{how mistakes increase as devices come near each other}).
%We also compute localization error of the user, and other microbenchmarks, such as robustness across users, impact of background sounds, impact of user mobility, etc.
%The next subsection presents the results.



\begin{figure*}[hbt]
\includegraphics[width=0.565\linewidth,trim= 0cm 0.5cm 0cm 1cm,clip=true]{figs/eval/method/photocoll_lowres.pdf}
\includegraphics[width=0.43\linewidth]{figs/eval/method/floorplan.pdf}
\caption{Four different rooms and a floor plan of the rooms with microphone icons show mic-array placements. These environments are multipath rich, as expected in real houses and offices.}
%\caption{Settings in 4 different rooms and a floor plan that includes 3 locations showcasing the diversity in room geometry, size and layout. Red circles highlight the mic-arrays that potentially co-locate with home appliances equipped with ASR/signal processing modules. These rooms represent typical domestic and enterprise settings including living rooms, canteen, and corporate meeting room. A selection of these mic-arrays collaboratively determine the user facing direction.}
\label{fig:rooms}
\end{figure*}

%-----------------------------------------------
%             Performance 
%-----------------------------------------------
    
\subsection{Performance Analysis}
$\blacksquare$ \textbf{Facing Direection Error}: 
Figure~\ref{fig:fd_dt_loc} shows the FDE and FIE errors for $2$, $4$, and $6$ devices.
The errors are derived from all the test configurations and sorted in increasing order.
The height of the bars indicate the FDE while their color indicates FIE.
For instance, with $4$ devices, the facing device is correctly identified in $XXX$\% of the test cases.
When errors occur, $XXX$\% of them exhibit an FIE of $1$, meaning the adjacent device is selected.
Moreover, observe that 2-device scenarios are not necessarily easier/better than $6$ because the user localization is better with $6$ devices, which aids in estimating the facing direction.
Results confirm this as well, showing a similar error distribution across different device densities.

\begin{figure}[hbt] %trim={<left> <lower> <right> <upper>}
\includegraphics[width=\columnwidth, trim={1em 0 3em 3em},clip]{figs/eval/performance/fd_dt_loc.eps}
%            \caption{\hl{I commented out a long caption}}
	\vspace*{-2em}
            \caption{Facing direction error in all tested cases employing 2, 4 and 6 number of devices. For each sub-figure, facing direction angular error is arranged in increasing order from left to right. We use 3 different colours to represent the number of missed devices by \name, i.e. the darker the colour is, the greater number of devices are in between the ground 
            truth and detected devices.}
\vspace{-1em}
%	In other words, the x-axis is test case index while y-axis depicts the error in degree. 
           \label{fig:fd_dt_loc}        
        \end{figure}


Figure \ref{fig:sep2acc} plots how angular separation between devices affect the inference accuracy.
%the accuracy of detecting the facing device.
The X axis represents angular ranges, e.g., the value $X=0$ means that the device adjacent to the facing device was located between $0$ to $40^{\circ}$ away.
For all test cases in which the adjacent devices were within $0-40^{\circ}$, the bars show the fraction of tests in which the facing device was accurately determined.
Naturally, the accuracy improves with increasing separation with the adjacent device.
This is intuitive because greater angular separation implies that the facing device has a proportionally stronger power compared to others.
This tends to improve the correlation with the human radiation pattern.
\new

Of course, this may not always be the case because large separation near the target devices naturally results in aggregation of the rest of devices, which can potentially lead to an aggregation of error in signal estimation. 
On the other hand, when there is only less than 10 degree between two devices, small user movements can affect accuracy.
After combining all these factors, {\name} achieves $XXX$\% accuracy even when the adjacent device is less than $40^{\circ}$ apart from the target device.
\new

        \begin{figure}[h]
            \centering
             \includegraphics[width=\columnwidth, trim={1em, 1em, 3em, 2.5em}, clip]{figs/eval/performance/sep2acc.pdf}
            %\includegraphics[width=1\columnwidth, trim={0,0,2em,2em}, clip]{figs/eval/performance/sep2acc.eps}
	    \vspace*{-1.5em}
            \caption{Estimation accuracy under different device separations, i.e. angle between the device user is facing
            and its adjacent device w.r.t the user.
            }
	    \vspace*{-1em}
            \label{fig:sep2acc}
        \end{figure}

\hl{A natural question is: in the face of errors, which device should respond to the voice command?
%One possibility is to use the output of {\name} as a filter, i.e., narrow down the possible devices.
One possibility is to delay the decision until the full command has been heard, and use the facing direction and command semantics jointly, to determine the intended device.}
For instance, if the facing device is either the TV or the adjacent floor light, and the voice command is ``Alexa, turn off in 10 minutes'', then the device that is currently ON can accept the command (another light that is in the opposite direction need not respond to this command).
Finally, if the TV and floor lamp are both ON, perhaps Alexa can clarify which device the user is referring to, by asking ``did you mean the TV or the floor lamp''.
\new

%We begin the evaluation of \name~with a close examination into how often error occurs and how bad the errors are in its inference, combining two aspects, i.e., the absolute angular error and the number of devices between the ground truth and the inferred devices, as shown in Figure~\ref{fig:fd_dt_loc}. 
%These results are produced from the entire dataset we collected for static users, grouped by number of active devices employed, i.e., 2, 4, and 6, corresponding to each sub-plot. 
%We use different shades of color to represent the number of devices in between ground truth and inferred devices by {\name}, and the y-value depicts the absolute angle between ground truth and detected devices, arranged in increasing order from left to right. 
%\new
%        
%    %   Discussion TODO
%We first observe from Figure~\ref{fig:fd_dt_loc} that in more than 350, 1600, 750 cases out of 572, 4608, 2824, \name~can correctly differentiate the facing device from 2, 4, and 6 devices. 
%The median of the absolute facing direction errors are
%\wally{0, 19, and 32} degrees for 2, 4, and 6 devices respectively, showing that \name~can reliably detect the facing device from the majority of test samples in 2 device cases while making only mistakes between devices with small angle separations when there are in total 4 or 6 devices.
%Meanwhile, the proportion of samples subject to errors $\le$60 degrees are \wally{79\%, 74\% and 77\%}\rui{check} for 2, 4, and 6 active devices respectively. This confirms that the absolute facing direction error does not depend on the number of devices. 
%\new


$\blacksquare$ \textbf{User Localization Error}: 
Figure ~\ref{fig:loc_all} plots the user localization error, as an outcome of AoA estimation and triangulation.
Results are again plotted for the $N=2$, $4$, and $6$ device settings.
The median errors are $0.7$m, $0.5$m, and $0.4$m, respectively.
The errors with $2$ devices are naturally higher since small AoA errors shift the intersection points during triangulation. 
With more devices, the system gets overdetermined, improving location accuracy.
With $6$ devices, for instance, around $90$\% of the test cases incur less than $1$m error.
Besides aiding in the facing direction problem, this user location can also be valuable to other applications that need indoor localization.
\new

%As an important building block of \name, localization accuracy is essential to the end-to-end performance of \name. Therefore, we investigate the localization error, i.e. euclidean distance between estimated and the true locations, in Figure ~\ref{fig:loc_all}. The results are obtained from the same dataset as in Figure~\ref{fig:fd_dt_loc}, and similarly organised in cases employing 2, 4, and 6 devices.
%    % Discussion TODO
%        As can be observed in Figure~\ref{fig:loc_all}, the median of the localization errors are \wally{0.7m, 0.5m, and respectively 0.4m} for 2, 4, 6 active devices.  
%        Intuitively, the localization error decreases significantly as the number of active devices increases, thanks to the increased number of AoA estimation that presumably makes the system more robust against noise and multipath effect. Building on top of reliable localization, the facing direction estimation of \name~does not decrease dramatically when the number of active devices increases.
%        Besides, we find that even with only $2$ active devices, a.k.a one intersection made from $2$ AoA inferences, the median localization error is less than 0.8m, which is sufficiently accurate for most of the indoor localization use cases.
%	\new
        
    \begin{figure}[h]
        \centering
        \includegraphics[width=0.8\columnwidth,  trim={2em, 0, 3em, 3em}]{figs/eval/performance/loc_cdf.eps}
	%\vspace*{-1em}
        \caption{Localization error in all tested cases, employing 2, 4, and 6 number of devices.}
	\vspace*{-1.2em}
        \label{fig:loc_all}
    \end{figure}

% Localization Error vs Facing direction error analysis Fig 6,7 (OL)
\iffalse
$\blacksquare$ \textbf{User localization error vs. facing direction estimation}: To further dissect {\name}'s performance and understand how localization error is translated into facing direction error, we observe in Figure ~\ref{fig:loc2fd} the distribution of localization error in every 20cm intervals (x-axis) and the corresponding facing direction error in degrees (y-axis). 
        \new
        
    % Discussion
        We can see that for speaker location errors lower than 1.5m, the facing direction error in both 4 and 6 devices settings increases as the location error.
        In other words, for dense device deployment, small localization error will likely to affect the facing direction estimation. Because there are more possible facing devices and \name~ needs to 
        accurately compensate fading caused by the user location.
        On the other hand, when there are only 2 devices active, the problem of differentiating from 2 devices the one faced by user is intrinsically easier, and hence tolerance of localization error appears to be larger. For location errors larger than 1.5m,
        the facing direction algorithm is dominated by the wrong location compensation rather than the radiation pattern, so the facing direction error of 2 devices setting is sometimes 
        even higher than the other settings.
	\new
        
        \begin{figure}[h]
            \centering
	    \vspace*{-1em}
            \includegraphics[width=\columnwidth, trim={0.2em, 0.5em, 4em, 3.4em}, clip]{figs/eval/performance/loc2fd_it0.eps}
	    \vspace*{-1em}
            \caption{Distribution of facing direction error v.s. localization error under 2, 4, and 6 active devices scenarios respectively.
            The dots mark the median value of the facing direction error for every $20$ cm user location error, and the error bars show the standard deviation.\rui{There's issue w this plot. y-value shouldn't be more than 200}%$XX$ and $XX$ percentiles. 
            }
	\vspace*{-1em}
            \label{fig:loc2fd}
        \end{figure}

    % Minimum angle separation v.s. Facing direction error
\fi
%-----------------------------------------------
%             Micro Benchmarks
%-----------------------------------------------

\subsection{Micro Benchmarks}

$\blacksquare$ \textbf{Incorporating P2P:} Although most of the home appliances would remain static once installed, we design a light-weight device-to-device localization algorithm as described in Section~\ref{sec:design} to relax the assumption on device location being known. Figure~\ref{fig:minis1}(a) illustrates the performance of \name\ incorporating the proposed P2P localization module. Note that with 2 devices it is impossible to obtain the location of both devices, we show here results only in 4 and 6 devices scenarios. When compared with Figure~\ref{fig:fd_dt_loc}, it is apparent that P2P localization will introduce minor errors to facing direction detection. Specifically, the median value of 4- and 6- device-deployment are respectively xx and xx lower as compared to when using true device locations.
\new

    Figure ~\ref{fig:minis1}(b) shows the P2P positioning result of different settings.
    Since the P2P algorithm only reports the relative direction between the devices,
    to calculate the positioning error, we scale the P2P estimation 
    using every device as the center, calculate the distance to the ground-truth and pick the minimum. 
    Choosing which device as center does not affect the following facing direction algorithm, 
    but help reader visualize the P2P accuracy. 
    \new

    % Discussion
    We find that as when there are $4$ anchor devices, the median P2P estimation
    error is less than $50$ cm, which in turn results in \rui{XX} more error in facing direction estimation. Relaxing the assumption of known device location is indeed at a moderate cost.  
 %position the devices when there are at least $4$ devices equipped with a speaker.
    \new
    
            \begin{figure}[h]
            \centering
            \includegraphics[width=\columnwidth]{figs/eval/bench/p2p_bench.pdf}
	    \vspace*{-1em}
            \caption{P2P localization error when using different number of devices and different subsets of anchor nodes.}%$XX$ and $XX$ percentiles. 
            \end{figure}
            

    $\blacksquare$ \textbf{User Mobility}: We test the proposed algorithm under mobile scenario, in which case the volunteer starts from the arbitary location and walks towards the target device while making the voice command. 
    Table ~\ref{tab:mobileNmic} shows the facing direction error distributions of mobile users in comparision with the static case. Note that due to space availability we collect mobile data from 4 rooms, while guaranteeing the settings are consistent with those of the user static case. 
    % Discussion
	The result confirms that the maximum difference in median errors between static and mobile users is 3 degrees among the scenarios employing 2, 4, and 6 devices. Hence we conclude that the impact of user's movement is negligible to \name.
\new
%\multirow{-2}{*}{\begin{sideways}TEST\end{sideways}}

\begin{table}[h]
        \begin{tabular}{c |c| c |c c}%{c|c|c|c}
            \toprule
	{}&{Num. of}  & \textbf{Mobile User}  &\multicolumn{2}{c}{\textbf{Static User}} \\
	{}&{Devices } &6 Mics  &6 Mics & 4 Mics   \\\midrule \midrule 
	\multirow{3}{*}{\rotatebox[origin=c]{90}{FDE}}
	&2   &  $0^{\circ}$   & $0^{\circ}$  & $0^{\circ}$ \\%\hhline{~-----}
	&4   &  $19^{\circ}$  & $7^{\circ}$  & $17^{\circ}$  \\%\hhline{~-----} 
	&6   &  $33^{\circ}$  & $21^{\circ}$ & $37^{\circ}$ \\\midrule
	\multirow{3}{*}{\rotatebox[origin=c]{90}{Loc. Err.}}
	%----mobile---6mics---4mics
	&2   &66cm &68cm   &190cm \\%\hhline{~-----} 
	&4   &59cm &49cm   &153cm \\%\hhline{~-----} 
	&6   &51cm &37cm   &143cm    \\\bottomrule
           
        \end{tabular}
        \vspace{0.5em}
       \caption{Median values for facing direction error and localisation error in benchmarking cases for  (a) static and mobile user, and (b) reducing the number of microphones per device.}
        \label{tab:mobileNmic}
	\vspace*{-1em}
\end{table} 


$\blacksquare$ \textbf{Number of Microphones}:
Figure ~\ref{fig:minis1} (c) shows the estimation results for enabling 4 and 6 microphones 
on the devices. The median errors are $XX$ and $XX$ for 4 and 6 microphones per device 
respectively.
\new

% Discussion
We find that the number of microphones per device will affect the AoA accuracy, which 
 will propagate to the user localization error. Moreover, one can observe a larger 
 error difference in 6 active devices scenario, because dense device deployment
requires accurate user location compensation. 
\new

$\blacksquare$ \textbf{$\widetilde{SNR}$}:
Figure ~\ref{fig:minis2} (a) shows the estimation error under different Signal-to-Noise Ratio ($\widetilde{SNR}$).
The $\widetilde{SNR}$ difference mainly come from 
(a) the ambient noise in the room, and (b) the loudness of the speech.
We categories the test samples according to the SNR calculated from the recorded signal.
\new

% Discussion
We find that the performance of \name\ is only marginally better under higher SNR scenario. In noisy environment of SNR down to 
$XX$ dB, \name\ can still achieve median error of $XX$ degrees.
\new

 %figure* and insert multiple figures in them ... and use the single caption (with (a), (b), (c)) to talk about them all .

    \begin{figure*}        
        \begin{minipage}{\textwidth}
            \includegraphics[width=.33\linewidth,  trim={1em, 0, 3em, 2.5em}, clip]{figs/eval/bench/snr2acc.pdf}
            % Same dummy as mobile, both compare between 2 settings XD
             \includegraphics[width=.33\linewidth,  trim={1em, 0, 3em, 2.5em}, clip]{figs/eval/bench/rad_patterns.eps}
             \includegraphics[width=.33\linewidth,  trim={1em, 0, 3em, 2.5em}, clip]{figs/eval/bench/fd_rad.eps}
            \caption{(a) Facing direction error grouped by $\widetilde{SNR}$. \rui{TO UPDATE}(b) 4 different radiation patterns employed for radiation pattern benchmarking.  (c) Distribution of facing direction error w.r.t each radiation pattern as shown in (b) when employ 2, 4, and 6 number of devices. 
            }            
            \label{fig:minis2}
        \end{minipage}%
    \end{figure*}
     

$\blacksquare$ \textbf{Radiation Pattern}:
To verify how the human speech radiation pattern affects the result, 
we use $4$ radiation patterns collected from different volunteers, 
as shown in Figure ~\ref{fig:minis2} (b).
Figure ~\ref{fig:minis2} (c) plots the estimation errors using each of these
$4$ radiation patterns to do pattern matching respectively. 
\new

% Discussion
Although there are small differences between these $4$ patterns, 
the overall shape is similar. As a result, the estimation results 
using these patterns are almost the same. 
This experiment confirms that a general human radiation pattern can be used
 for pattern matching. 
\new


    $\blacksquare$ \textbf{Computation Time}:
    Table ~\ref{tbl:comp} shows the median computation time under different scenarios. 
    The median computation of our algorithm is 0.35s for generating results presented in Fig.\ref{fig:fd_dt_loc} on a Raspberry Pi 4 with quad core Cortex-A72 (ARM v8) 64-bit SoC @ 1.5GHz with 4GB  SDRAM.
     %Linux desktop device with 125GiB System memory Intel(R) Core(TM) i7-7800X CPU @ 3.50GHz. %\rui{There is certainly dilemma between accuracy and computation time. We envision this to be trivial as the maximum computation time in call cases is 1.3s.}
\new
    \begin{table}[t]
        \begin{tabular}{c c c c}%{c|c|c|c}
            \toprule
            Num. of active devices & 2   & 4   & 6    \\ \midrule            \midrule
            P2P devices localization & XX  & XX  & XX   \\ \hline
	    Facing device estimation &153 &305 & 451 \\ \bottomrule
%            Facing device estimation & 279 & 780 & 1277 \\ \bottomrule %overall mean 0.78s
        \end{tabular}
        \caption{Median computation time of \name\ in micro-seconds using different number of active devices.}
        \vspace*{-2em}
        \label{tbl:comp}
    \end{table}
 
    %Rui: for our notes the time increases as the number of devices involved. 
    %mean computation time in sec for 2, 4, 6  devices are respectively 0.2795752698482748 0.7809380368328528 1.2785372068439225
    % median computation time in sec for 2, 4, 6  devices are respectively 0.27890515327453613 0.7800725698471069 1.2773441076278687
    %overall mean  0.9335383917738336  median  0.7816259860992432
    % min 0.28s and max 1.3s for 2, 4, 6 



==> tex/eval_rui.tex <==
\begin{table}[h]
        \begin{tabular}{c |c| c |c |c}%{c|c|c|c}
            \toprule
	{}&{Num. of}  & \textbf{Mobile}  &\textbf{Static} &\textbf{Static} \\
	{}&{Devices } &6 Mics  &6 Mics & 4 Mics   \\\midrule \midrule 
	\multirow{3}{*}{\rotatebox[origin=c]{90}{FDE}}
	&2   &  $0^{\circ}$   & $0^{\circ}$  & $0^{\circ}$ \\%\hhline{~-----}
	&4   &  $11^{\circ}$  & $0^{\circ}$  & $20^{\circ}$  \\%\hhline{~-----} 
	&6   &  $15^{\circ}$  & $8^{\circ}$ & $37^{\circ}$ \\\midrule
	\multirow{3}{*}{\rotatebox[origin=c]{90}{Loc. Err.}}
	%----mobile---6mics---4mics
	&2   &66cm &68cm   &190cm \\%\hhline{~-----} 
	&4   &59cm &49cm   &153cm \\%\hhline{~-----} 
	&6   &51cm &37cm   &143cm    \\\bottomrule
           
        \end{tabular}
        \vspace{0.5em}
       \caption{Median values for facing direction error and localisation error in benchmarking cases for  (a) static and mobile user, and (b) reducing the number of microphones per device.}
        \label{tab:mobileNmic}
	\vspace*{-1em}
\end{table} 

    \begin{table}[t]
        \begin{tabular}{c c c c}%{c|c|c|c}
            \toprule
            Num. of active devices & 2   & 4   & 6    \\ \midrule            \midrule
            P2P devices localization & {-}  & 578  & 631   \\ \hline
	    Facing device estimation &153 &305 & 451 \\ \bottomrule
%            Facing device estimation & 279 & 780 & 1277 \\ \bottomrule %overall mean 0.78s
        \end{tabular}
        \caption{Median computation time of \name\ in micro-seconds using different number of active devices.}
        \vspace*{-2em}
        \label{tbl:comp}
    \end{table}
 

==> tex/eval_samsung__.tex <==
% NO LONGER USED 
%This is a temporary tex separated from eval.tex for Rui/ Abhinav to edit to avoid conflict
% For the following three benchmarks, we requested help from you and feel free
% to modify anytime

$\blacksquare$ \textbf{Number of Microphones}:
Figure ~\ref{fig:microphone} shows the estimation results for enabling 4 and 6 microphones 
on the devices. The median errors are $XX$ and $XX$ for 4 and 6 microphones per device 
respectively.
\new

% Discussion
We find that the number of microphones per device will affect the AoA accuracy, which 
 will propagate to the user localization error. Moreover, one can observe a larger 
 error difference in 6 active devices scenario, because dense device deployment
requires accurate user location compensation. 
\new

$\blacksquare$ \textbf{SNR}:
Figure ~\ref{fig:SNR} shows the estimation error under different Signal-to-Noise
Ratio (SNR) scenarios. The SNR difference might come from 
(a) the ambient noise in the room, and (b) the loudness of the speech
We categories the test samples according to the SNR calculated from the recorded 
signal
\new

% Discussion
We find that the performance of \name\ is better under higher SNR scenario,
 but the difference is not very large. In noisy enviroment of SNR down to 
$XX$ dB, \name\ can still achieve median error of $XX$ degrees.
\new
    \begin{figure*}        
        \begin{minipage}{.33\textwidth}
            \includegraphics[width=\linewidth,  trim={1em, 0, 3em, 2.5em}, clip]{figs/eval/bench/snr2acc.eps}
            % Same dummy as mobile, both compare between 2 settings XD
            \caption{Facing direction error grouped by $\widetilde{SNR}$ .
            \wally{should we show localization error?}}
            \label{fig:SNR}
        \end{minipage}%
        \hfill
        \begin{minipage}{.33\textwidth}
            \includegraphics[width=\linewidth,  trim={1em, 0, 3em, 2.5em}, clip]{figs/eval/bench/rad_patterns.eps}
            % Same dummy as mobile, both compare between 2 settings XD
            \caption{We run experiments on these 5 different radiation patterns.}
            \label{fig:radpattern}
        \end{minipage}%
        \hfill
        \begin{minipage}{.33\textwidth}
            \centering
            \includegraphics[width=\linewidth,  trim={1em, 0, 3em, 2.5em}, clip]{figs/eval/bench/fd_rad.eps}
            \caption{Distribution of error w.r.t each radiation pattern as shown in \ref{fig:radpattern} when employ 2, 4, and 6 number of devices.}
            \label{fig:fd_rad}
        \end{minipage}%
    \end{figure*}

$\blacksquare$ \textbf{Radiation Pattern}:
To verify how the human speech radiation pattern affects the result, 
we use $5$ radiation patterns collected from different volunteers, 
as shown in Figure ~\ref{fig:radpattern}.
Figure ~\ref{fig:fd_rad} plots the estimattion errors using each of these
$5$ radiation patterns to do pattern matching respectively. 
\new

% Discussion
Although there are small differences between these $5$ patterns, 
the overall shape is similar. As a result, the estimation results 
using these patterns are almost the same. 
This experiment confirms that utilizing a general human radiation pattern
 for pattern matching does not affect the results.
\new


==> tex/limitations.tex <==
\section{Limitations and Discussions}

%$\blacksquare$ \textbf{The Absence of LoS Paths}:
%A complete absence of LoS path from the user to a device will produce incorrect results. 
%However, the presence of even a weak LoS component is sufficient for our purposes.

%$\blacksquare$ \textbf{Assuming LoS paths between devices}:
%Our P2P algorithm assumes reasonably strong LoS paths between the anchor and other devices. 
%Acoustics-absorbing obstacles between these devices can violate this assumption, and if enough of such links are obstructed, the device localization results can be derailed.
%%When there are obstacles between the devices,
%% the P2P localization might not converge and report a random 
%%results. 
%Fortunately, since we can estimate the exact channels between the devices (since the speakers can play a known preamble), we can infer whether
%there is a LoS path from the channels accordingly.  
%Thus, when failure ensues, {\name} can at least be self-aware. 


$\blacksquare$ \textbf{Single-microphone Devices:} 
A device $D_{s}$ may be equipped with a single microphone, hence cannot contribute its AoA for localization/triangulation.
However, so long as it has an embedded speaker, it can participate in P2P device localization, and its locations can be inferred.
Since user triangulation does not need all the devices, the user's location can also be computed without $D_{s}$'s location.
Now, when estimating the facing direction, it may be possible to identify that the user is facing $D_{s}$ from the correlation patterns.
We have left such analysis and algorithms to future work.
\new

$\blacksquare$ \textbf{Self Interference:} 
Many devices -- such as refrigerators, A/C machines, TVs, water faucets, etc. -- produce sounds as an outcome of their normal operation.
This sound will pollute the recorded voice signals and could cause the LoS power estimates to become erroneous.
We have not tested such cases in this paper.
However, given these sounds are \hl{typically stationary random processes}, their power profile may not change significantly.
Thus, it should be possible to characterize this noise floor (before the start of the command) and subtract it from the estimated LoS signal.
\new

%Some smart devices may be equipped with a single microphone, hence cannot contribute their AoAs for localization/triangulation.
%% Such devices cannot provide AoA results when localizing the user, 
%However, they can still contribute to source signal estimation and detect whether 
%the user is talking to them with other devices as well.
%Moreover, if they are equipped with a speaker, they can serve as the
%anchor devices in p2p algorithm estimating its own location.

$\blacksquare$ \textbf{Online learning}:
Many locations and surroundings of the devices may remain unchanged over time, suggesting strong channel coherence between two voice commands (from the same location). 
The {\name} system should learn from the past results and refine both user location and channel estimates. 
This work leaves this opportunity untapped.
\new

%$\blacksquare$ \textbf{Strong reflectors}:
%\name\ estimates source signal by delay-and-summing
%all the received signals. However, if there are strong reflectors 
% around few devices, the corresponding channels will 
% contain strong multipath components, and summing 
%signals from those devices might not help create the
%clean estimated source signal. Device selective delay-and-sum 
%might be one of the possible ways to improve channel estimation
%performance.

$\blacksquare$ \textbf{Leverage the full voice command}:
We have used only the short wake-up word to localize and infer the facing direction. 
While the user is speaking the rest of the voice command, we utilize that time to complete the facing direction computation.
If devices are more powerful, a longer part of the voice command could be used.
Longer signals (over stable channels) will help average out the white-sense stationery noises, likely refining the channel estimation results.

%This opportunity could be tapped in real cases
%Accordingly, in real cases if the full voice commands are available, 
% we can use longer signals to calculate the channel and the 
%estimation results are likely to improve. 

 


==> tex/related.tex <==
\section{Related Work}

\textbf{Inferring Pose and Facing Direction.} 
To the best of our knowledge, facing direction and pose estimation has mostly been studied in computer vision, where the challenge is to estimate poses using a single camera \cite{mariani2004face,yasumoto2000face, fanelli2011real, pateraki2014visual}. 
We believe this paper may be the first study towards inferring facing direction from (unknown) human voice signals. 
Of course, much work exists on human radiation patterns, and in using voice for ranging \cite{peng2007beepbeep}, localization, motion tracking \cite{mao2019rnn,mao2016cat,smith2004tracking, yun2017strata, zhang2012swordfight}, etc. 
Radiation patterns (of antennas) have also been used for RF localization and sensing\cite{xiong2013arraytrack, wu2012csi, bocca2013multiple, kotaru2015spotfi, wang2017mfdl, karanam2018wifiTrack, sen2013avoiding, mariakakis2014sail, zheng2014CSI, vasisht2016decimeter}, however, source signals are often known in such systems.
Facing direction is difficult due to unknown source signals that vary slightly over adjacent facing directions.
%RF communication systems, while acoustic signals vary distinctly for localization and motion tracking.
%With acoustic facing direction, {\name} is faced with the worse of both worlds -- unknown source signals, that change slightly over adjacent facing directions. 
\new

\textbf{AoA Estimation and Beamforming.}
Literature in beamforming and AoA is extremely mature~\cite{dokmanic2013roomshape, dokmanic2015thesis, ribeiro2010turning,anManocha2018reflection, anManocha2019diffraction}. 
For AoA detection one of the most commonly used algorithm is GCC-PHAT~\cite{knapp1976generalized, brandstein1997robust, benesty2004time, freire2011doa, van2012time}.
Recent years have also seen subspace based algorithms (e.g., MUSIC and ESPRIT) for AoA estimation \cite{roy1989esprit, schmidt1986music, sit2012direction, tang2014doathesis, xu2017weighted},
although they assume multiple uncorrelated source signals. %that the signals captured by different microphones are uncorrelated, which is not the case for GCC-PHAT. 
Acoustic AoA and filtering have also been used in new types of imaging applications \cite{mao2018aim,mao2019mobile}. 
{\name} borrows from this literature to bring together the complete system -- we do not contribute here.
\new

\textbf{Acoustic Localization and Sensing.}
User localization using acoustic signals have also been well explored in the literature. 
Various approaches have been studied, including elapsed time of arrival~\cite{peng2007beepbeep}, 
exploiting wide-band signal and microphone array \cite{dokmanic2013roomshape, dokmanic2015thesis}, 
combining AoA determined by iterative align-and-cancel algorithm and inferred geometry of the closest reflector from multiple voice commands~\cite{shen2020voloc}, and 
by estimating room geometry and the time difference of arrival (TDOA)~\cite{dokmanic2013roomshape, dokmanic2015thesis, ribeiro2010turning, anManocha2018reflection, anManocha2019diffraction}. 
%Similarly, studies have also explored solving the problem of user localization by RF signals, which require Wi-Fi access points or dedicated RF sensors 
Facing direction is a somewhat complementary problem; localization is necessary but not sufficient to solve facing direction.
\new

\textbf{Blind Channel Inference (BCI) and De-reverberation.} 
BCI a well known problem in wireless communication, medical imaging, and signal processing. 
Classical information theorists approach this problem via statistical methods such as second-order \cite{tong1994blind} and cyclostationary \cite{tong1991new} statistics, or sub-space based methods \cite{muquet2002subspace}.
Also, work on speech de-reverberation has proposed methods that estimates the source signal using linear prediction model, which employs gradient descend on the channel using Kurtosis of the frequency spectrum as an objective function \cite{gillespie2001speech}.
Such techniques, while applicable in principle, are impractical due to the time and CPU budget in voice assistants.
{\name}'s contribution is in operating at the intersection of unique application specific constraints and opportunities.




%
%%- To the best of our knowledge, facing direction detection of the user has not yet been discussed in acoustic research.\\
%%- In this section, we will discuss some most significant acoustic signal processing techniques appeared in previous work that are relevant to our paper.\\
%
%%acoustic sensing, ranging, localisation etc. 
%\textbf{Acoustic Sensing: Ranging, AoA, Localisation and More} %tracking and imaging
%The vast availability of acoustic information thanks to the ubiquitous microphones and speakers in commodity mobile devices led to a number of dimentions acoustic sensing technology including ranging \cite{peng2007beepbeep}, AoA detection and user localisation \cite{dokmanic2013roomshape, dokmanic2015thesis, ribeiro2010turning,anManocha2018reflection, anManocha2019diffraction}, motion tracking \cite{mao2019rnn,mao2016cat,smith2004tracking, yun2017strata, zhang2012swordfight}, and imaging \cite{mao2018aim,mao2019mobile}. 
%\new
%
%GCC-PHAT based AOA detection has been widely employed \cite{knapp1976generalized, brandstein1997robust, benesty2004time, freire2011doa, van2012time}. While with the premise that signals captured by different antenna/microphone elements are uncorrelated, subspace based algorithm such as MUSIC and ESPRIT have been used in AoA estimation \cite{roy1989esprit, schmidt1986music, sit2012direction, tang2014doathesis, xu2017weighted}.
%% MUSIC devides the spatial covariance matrix (SCM) to source subspace and noise subspace by the eigenvalue decomposition and then estimated the TDOA by searching the steering vectors orthogonal to the noise subspace.
%\new
%
%Taking a step forward from AoA, a few work in literature address localisation of the sound source. For example, Peng \emph{et al.} develop a seminal device-to-device acoustic ranging system based on elapsed time between the time-of-arrivals, leveraging microphones and speakers in commercial off-the-shelf devices~\cite{peng2007beepbeep}. 
%\new

%single speaker and mic per device, no synchronisation assumptions
%\\- Room acoustics is one major approach to indoor user localisation \cite{dokmanic2013roomshape, dokmanic2015thesis, ribeiro2010turning, anManocha2018reflection, anManocha2019diffraction}. 
%Dokmanic \emph{et al.} propose algorithm to infer the shape of the room by exploiting a carefully designed wide-band signal and microphone array \cite{dokmanic2013roomshape, dokmanic2015thesis}. VoLoc \cite{} propose an \emph{unknown} sound source localisation algorithm using a single microphone array that combines AoA determined by iterative align-and-cancel algorithm and inferred geometry of the closest reflector from multiple voice commands. The algorithm performs accurate user localisation, but assumes the presence of a strong reflector (e.g. wall) near the device. 
%Ribeiro \emph{et al.} employ a loudspeaker integrated with a microphone array that emits a probing sound in order to estimates height of the ceiling and locations of the walls, and then devise a maximum likelihood based algorithm to detect sound source~\cite{ribeiro2010turning}. This work, however, assumes rectangular conference room and the microphone sitting in a carefully chosen position around center of the room. 
%In summary, sound source localisation algorithms based on room geometry obtained from microphone signals \cite{dokmanic2013roomshape, dokmanic2015thesis, ribeiro2010turning} rely on the first order echo to be clearly captured, which in turn requires specific room shapes and microphone position. %add voloc reference
%Authors in \cite{anManocha2018reflection} use advanced sensors to construct point cloud streams for subsequent SLAM module to produce an octree-based occupancy representation of the room environment, followed by computing direct and reflected acoustic paths based on time difference of arrival (TDOA) and the room properties to estimate the sound source position. 
%Similarly, the work presented in \cite{anManocha2019diffraction} exploits the diffraction properties of sound waves to localise sound source via NLOS paths. 
%Methods proposed in \cite{anManocha2018reflection, anManocha2019diffraction}, however, require Kinect and Laser scanner to generate room representation. Meeting such requirements are hardly feasible outside of robotics lab environment. 
%Facing direction estimation, on the other hand, has only been thus far studied in computer vision, which require at least one camera \cite{mariani2004face,yasumoto2000face, fanelli2011real, pateraki2014visual}. 
%\new

%wifi localisation
%\textbf{RF Localisation} Most of the existing RF localisation technologies requires multiple Wi-Fi access points or dedicated RF sensors \cite{xiong2013arraytrack, wu2012csi, bocca2013multiple, kotaru2015spotfi, wang2017mfdl, karanam2018wifiTrack} 
%Among these, some require absolute phase measures on a software defined radio~\cite{xiong2013arraytrack}, which are not always available, and others calls for intense calibration either to fingerprint target locations \cite{wu2012csi}, or to calibrate CSI phase offset \cite{wang2017mfdl}. 
%Single AP solutions including \cite{sen2013avoiding, mariakakis2014sail, zheng2014CSI, vasisht2016decimeter} mostly require users to move to multiple locations to mimic the presence of multiple access points~\cite{sen2013avoiding, mariakakis2014sail, zheng2014CSI}. 
%Wi-Fi localisation requires user to carry a device, and study has shown that localisation feature has negative impact on Wi-Fi throughput~\cite{vasisht2016decimeter}.
%\new


%Previous study show that human radiation pattern persists \cite{dunn1939radpattern} and we will exploit this fact.


==> tex/sysdesign.tex <==
\section{System Design}
\label{sec:design}

\begin{figure*}
\includegraphics[width=\linewidth]{figs/blockDiagram2.pdf}
\caption{System architecture of CoDIR: Each device runs the AoA Estimator locally and forwards the AoA and the voice signals to the leader device (cloud, edge, or a leader device). The leader performs signal processing across all the signals, inferring the user location and facing direction.}
\vspace{-0.1in}
\label{fig:system}
\end{figure*}

Figure \ref{fig:system} shows the end-to-end system pipeline.
Each device $D_i$ activates with the wake-word like ``Alexa'' and runs an \texttt{AoA Estimator} locally to derive the angle $\theta_{i}$ from which it receives the signal. 
The recorded signal and the AoA are forwarded to a leader device (either the cloud, an edge router, or one of the voice assistants) by all other devices.
The leader uses the AoAs to first triangulate the user's 2D location.
Since \texttt{User Triangulation} requires the device locations, the leader relies on a \texttt{P2P Device Localization}, which runs during the setup time, to infer the device configuration.
The result of triangulation yields the user's distance to each of the devices -- these distances and the raw signals are then forwarded to the {\name} algorithm.
As described in Section \ref{}, the algorithm outputs the target device $k$ and user location $L_{<x,y>}$.




\subsection{P2P Device Localization}
During installation, and periodically after that (perhaps every night or when some devices have moved) the {\name} system runs a device localization protocol.
The electronic speaker embedded in each voice assistant broadcasts a short chirp; other devices overhear the chirp and compute their own AoAs using the AoA Estimator as discussed below.
\new

\textbf{AoA Estimator.}
AoA estimation is performed locally for parallel operations (i.e., saves time at the leader device).
Since only the LoS angle is necessary, we adopt the well-established generalized cross-correlation phase transform (GCC-PHAT) algorithm \cite{knapp1976gcc}. This algorithm aims to compute time delay between two signals. In order to do this, it performs the generalized cross-correlation between the two signals and takes the location of the peak of the cross-correlation values $G$ to find the time delay. We extract the correlation values $G$ from this algorithm for our AoA computation. 
\new

The standard implementation of GCC-PHAT based AoA estimation picks the microphone pair that subtends the largest acute angle to the direction of the signal. We modify this to compute the AoA for $\frac{M}{2}$ pairs, i.e., the diagonally opposite ones. More specifically, we take signals from each microphone pair $p \in [1,\frac{M}{2}]$ of device $D_i$ and compute cross-correlation values $g^p_i$ for that pair. 
Since microphones on a given device are located very close to each other, GCC-PHAT could not give us correlation values at a fine AoA granularity.
Therefore, we interpolate the correlation values $g^p_i$ at a granularity of $1^{\circ}$ within the range of $[1,2\pi]$.
Once this is done for each microphone-pair on a device, the interpolated cross-correlation values $g^p_i$ for all pairs are combined by averaging over each degree, which we define as $\hat{g}^p_i$. 
Finally, the AoA $\theta_i$ is obtained by taking the position of the peak of the cross-correlation values $\hat{g}^p_i$. More formally, this is done as:
\begin{displaymath}
\theta_i = argmax_{\theta} |\hat{g}^p_i|
\end{displaymath}


Once the AoAs are computed by each device, they are forwarded to the leader device, which now runs the following steps:

\textbf{Step1.} Source signal $x^i$ triggered by device $D_i$ and signals $x^i_{jk}$ received by microphones $k \in [1,M]$ of all other devices (i.e., $j \in [1,N]$  with $j \ne i$) are used to calculate the received channel $h^i_{jk}$ as:
\begin{displaymath}
h^i_{jk}=IFFT(\frac{x^i_{jk}}{x^i})
\end{displaymath}

\textbf{Step2.} We then calculated the AoA $\theta_{ij}$ from device $D_i$ to device $D_j$ using the received channel $h^i_{jk}$ estimated in the previous step. This is computed as:  
\begin{displaymath}
\theta_{ij}=gccphat(h^i_{jk}|_k)
\end{displaymath}
In order to compute $\theta_{ij}$ we pass $h^i_{jk}$ to the AoA Estimator module, which uses GCC-PHAT for computing the angle of arrival for signal based on the received channels by opposite pairs of microphones.   
\new

\textbf{Step3.} Now, all the unreliable $\theta_{ij}$ are removed to reduce noise. A $\theta_{ij}$ is considered as unreliable if it is far from $\theta_{ji}+180^\circ$. Note that $\theta_{ji}$ is calculated when device $D_j$ is used as an anchor device.
\new

\textbf{Step4.} Finally, the locations $L^{D_i}_{<x,y>}$ of devices are optimized as:
\begin{displaymath}
argmin_{\mathbf{x, y}} \sum_{i,j} |angle(L_{<x,y>}^i - L_{<x,y>}^j)-\theta_{i}^{j}|
\end{displaymath}


It is worth noting that the locations of devices estimated by this component are not the actual positions of devices with reference to the floor plan. Instead, the estimated location of each device is in reference to other devices. However, if required by any app, it is possible to extract the coordinates of device in reference to the floor plan. To do this, the app would need the floor plan of the building and could ask the user to stand at some specific reference points on the map to speak the wakeup work so that the devices could figure out their location with respect to that point. 


\subsection{User Triangulation}
The two modules (P2p device localization and AoA estimator) discussed above have computed each device's location and the voice signal's angle of arrival (AoA) at each device.
This implies that triangulation is feasible (i.e., rays emanating from each device in the house or office).
Ideally, the rays should intersect at a single location -- the user location. 
In reality, AoA and P2P location errors cause the rays to deviate, producing many points intersection points.
To cope with outliers, we perform a density based clustering using DBScan \cite{ester1996density}. 
\new

DBScan a non-parametric density-based clustering algorithm. Given a set of points, it groups together the points that are closely packed together and eliminates outliers by removing the low-density groups. In order to perform this clustering, we set the minimum density of the cluster as 2 points and the maximum cluster radius is set to $1$m.  
The cluster with the highest number of points is retained, and the rest are eliminated. 
The centroid of this cluster is declared as the user's location $L_{<x,y>}$. 
In the case when no cluster is formed by DBScan (i.e., when the points are sparsely distributed in the space), we take the centroid of all points as the user's location $L_{<x,y>}$.






















%\section{System Design}
%\label{sec:design}
%
%
%In this section we present the proposed system for predicting a speaker's facing direction in the context of multiple voice assistants. Specifically, we present the end-to-end system design that takes $x_{i,j}$ (where $i \in [1,N]$ and $j \in [1,M]$) and notifies the device $k$ which is predicted to be the one a user is speaking to. Overall, the system comprises of three key components: \textit{AoA Estimation}, \textit{P2P Device Localization}, and \textit{User Triangulation}, which help the \textit{CoDIR} component to predict the facing device. 
%
%In Figure~\ref{fig:system} we present the architecture of the proposed system. The system first setup itself by estimating the location of all devices ($D_{<x,y>}^{i}$) through the P2P Device Localization component that stores these locations for later use by the system. Once this is done, the system is ready for predicting the user's facing direction. In order to do so, the signals ($x_{i, 1:M}$ from all microphones of each device $i \in [1:N]$ are passed to AoA Estimation component for computing the AoA ($\theta_i$) of the speaker with respect to device $i$. Now these AoAs along with the source signals $x_{i, j}$ are transmitted to the leader device that is responsible for performing facing direction prediction and notifying the predicted device. The User Triangulation component uses these signals along with the location of all devices $D_{<x,y>}^{i} $ (obtained from P2P Device Localization component) to compute the user's location ($L_{<x,y>}$. Finally, the source signals, deice locations and the user's location are passed to the CoDIR component to predict the device to which the user is speaking to. Once a prediction is made, the leader device notifies the predicted one to perform the action for user's command. 
%  
%
%\subsection{AoA Estimator}
%
%The AoA Estimator component is responsible for computing the AoA of the source signal to the device. It is the first component of the system and is available on each device for enabling efficient distributed computation. To estimate the AOA $\theta_i$ on a device $D_i$ it exploits signals $S_{i,j}$ from all $M$ microphones, where $j \in [1, M]$. As the first step, diagonal pairs of microphones are selected, by assuming that the system knows the position of microphones on each device. Let us call these pairs as $P \in [p_1, p_2, ..., p_{M/2}]$. Now each pair of source signals ($S^1_{p_k}$ and ($S^2_{p_k}$) belonging to a pair $p_k \in P$ is used to compute AoA based on GCC-PHAT algorithm~\cite{}. Since microphones on ASR devices are located very close to each other, GCC-PHAT could not give us correlation values for a fine granularity of AoA. Therefore, we perform the interpolation to compute the correlation values at a granularity of $1\circ$, which we define as $G_{k,\theta}$ where $\theta \in [1:180]$. 
%
%
%Once the above task is performed for each pair of microphones of a device $D_i$, the GCC-PHAT values for iterations are cobined by taking the average over each degree. Finally, the AoA $\theta_i$ for source signal to device $D_i$ is obtaineded as:
%\begin{displaymath}
%argmax_{\theta} |G_{k,\theta}|
%\end{displaymath}
%
%
%
%\subsection{P2P Device Localization}
%
%
%The P2P Device Localization component is used by the system to estimate the location of all devices. To do this, an anchor device $D_i$ transmits a signal $S^i$, and microphones of all other devices receive a signal $S^i_{j,k}$ (where $k$ is the microphone of a device $D_j$). This is repeated by selecting a few devices as anchor devices in order to get a reliable estimate of device location. Once this is done, signal collected in each iteration are passed to the leader device, which entails the P2P Device Localization component for estimating the location of all devices by performing the following four steps. 
%
%
%\textbf{Step1.} Signals $S^i_{j,k}$ received by a device $D_j$ are used to calculate the channel as:
%\begin{displaymath}
%h^i_{j,k}=IFFT(\frac{S^i_{j,k}}{S^i})
%\end{displaymath}
%
%
%\textbf{Step2.} We then calculated the AoA from device $D_i$ to device $D_j$ using the signals received by the microphones of $D_j$. This is computed as: 
%\begin{displaymath}
%\theta_{ij}=gccphat(h^i_{j,k}|_k)
%\end{displaymath}
%
%
%\textbf{Step3.} Now, all the unreliable $\theta_{ij}$ are removed to reduce noise. A $\theta_{ij}$ is considered as unreliable if it is far from $\theta_{ji}+180^\circ$. Note that $\theta_{ji}$ is calculated when device $D_j$ is used as an anchor device.
%
%
%\textbf{Step4.} Finally, the locations $L^{D_i}_{<x,y>}$ of devices are optimized as:
%
%\begin{displaymath}
%argmin_{\mathbf{x}} \sum_{i,j} |angle(L_{<x,y>}^i - L_{<x,y>}^j)-\theta_{ij}|
%\end{displaymath}
%
%
%
%
%
%
%
%
%\subsection{User Triangulation}
%
%
%
%The User triangulation component is used to localise the user by exploiting the AoAs $\theta_i$ received from device $D_i$ (where $i \in [1,N]$) and location of devices (i.e., $L^{D_i}_{<x,y>}$) obtained from P2P Device Localization component. A project of an AoA is drawn from the position of each respective device and all intersection points of these AoAs are computed. Since there could be possible outlier that can bring error to the estimation of the user's location. We perform a density-based clustering on all intersection points. We use DBScan~\cite{} clustering algorithm with the parameters such that each cluster contains at least 2 points and the maximum distance is 1 meter. We select the cluster that has the highest number of points and eliminate other points. Finally, the centroid of remaining points is computed, which is considered as the user's location $L_{<x,y>}$. 
%
%
%
%
%
%%\subsection{Facing Direction Prediction}
%
%
%
%
%
%

